On the Linear Algebraic Monoids Associated to Congruence of Matrices

This paper discusses the generalized congruence equation $X^tAX=B$, for $X \in M_n(k)$ over any field $k$, through the action of monoid $Sol_A \times Sol_B := \{X \ | \ X^tAX = A\} \times \{X \ | \ X^tBX = B\}$. We have completely characterized for what matrices $A$, the monoid $Sol_A$ is a Lie group. We have given the structure of the Lie group $Sol_A$ and $Sol_{A^2}$, and their Lie algebras when $A$ is $n \times n$ nilpotent matrix of nilpotency $n$. In this case, we have also proved that the invariants of $Sol_A$ for any $n$, and $Sol_{A^2}$ for $n$ even, are finitely generated.

==> temp.tex <==

\section{Introduction}
Two square matrices $A,B$ with coefficients over a field $k$ are called congruent if there is an invertible matrix $P$ of appropriate dimension such that $A=P^tBP$. The question of the existence of such an invertible matrix, when two matrices $A,B$ are provided, is called the congruence problem of matrices. It is an important classical problem in mathematics, with a vast and interesting history \cite{Teran_history}. This question is solved completely through the classification of the matrix pencils, $P(A,B)=\lambda A + \mu B$, where two such pencils $P(A,B)$ and $P(A',B')$ are called equivalent if there are invertible matrices, $\alpha, \beta$ of appropriate size such that $P(A,B)=P(\alpha A'\beta, \alpha B'\beta)$. Classification of pencils up to equivalence is an important problem in linear algebra. It is a particular case of the class of problems called ``simultaneous equivalence" or ``simultaneous similarity"of matrices \cite{Simultaneous}. The problem of simultaneous similarity or simultaneous equivalence is difficult, and a particular case of this problem is the classification of matrix pencils. The matrix pencil classification problem has been fully solved by the cumulative efforts of several authors spanning the last century. Namely, the classification of singular matrix pencils by Kronecker \cite{Aitken}. A special class of matrix pencils is the class of ``palindromic pencils" namely, the pencils $\lambda A + \mu A^t$, a classification of such pencils gives an answer to the congruence problem through the canonical forms of matrix pencils \cite{Teran_history}. These canonical forms for the palindromic pencils are not easy to work with as the canonical form is a direct sum of six types (\cite{Aitken}) of matrices. This resulted in several articles with further simplification approaches to this problem. There are currently four types of canonical forms given for the solution of the equivalent pencil problems (each of these give rise to canonical forms for the congruence problem) but all of these are of a similar essence. 

In this article, we look at the congruence problem differently and aim to arrive at a group theoretic or geometric solution to this problem. To a matrix, we associate a monoid $Sol_A$, which is the collection of all square matrices $X$, singular or non-singular, such that $X^tAX=A$.  We observe that two matrices $A,B$ are congruent to each other if and only if there is an inner automorphism of $GL_n$ that takes the monoid $Sol_A$ to $Sol_B$ isomorphically. This naturally shows that one can arrive at a classification, not through the matrix pencil approach but through classifying these monoids up to inner-automorphisms. As a first step towards this solution, one must understand these monoids' structure. To understand the linear algebraic monoid \cite{putcha}, one must first understand the monoid's group of invertible elements. In our case, the group $GL_n \cap Sol_A$ for a given matrix, $A$ has to be understood. 

************************************************************************************************************************
For symmetric matrices $A$ and $B$, the solution is provided by Sylvester's theorem on inertia. If $A$ and $B$ are skew-symmetric, orthogonal transformations reduce both matrices to canonical forms used to classify skew-symmetric pairs. The general solution to this problem has attracted many mathematicians. A typical approach to the congruence problem is to express any matrix $A$ as a unique sum of two matrices - one symmetric and the other skew-symmetric, i.e., $A=A_1+A_2$. Then, the focus shifts to the action of the orthogonal group on $E\times F$, where $E$ represents the vector space of symmetric matrices and $F$ represents the vector space of skew-symmetric matrices. After classifying the orbits of this action, it can be shown that the obtained invariants provide invariants for matrix $A$. These invariants are known as canonical classes for matrix $A$. Using these canonical classes, the congruence question is completely solved over complex numbers (or any algebraically closed field).

In a series of papers, Williams \cite{W1},\cite{W2} systematically studied the congruence problem for finite fields, as well as for both $\mathbb{R}$ and $\mathbb{C}$. Moreover, Horn, Sergeichuk, and others have published numerous papers on canonical forms for congruence and $^*$congruence matrix problems ($X^tAX=B$) \cite{W3}\cite{W4}\cite{Horn1}\cite{Horn2}. The projective congruence question ($X^tAX=\lambda B$ for any $\lambda \in K^{*}$) has also garnered interest, with recent work by Edelman et al. focusing on the structure of solutions to the matrix equation $X^tAX=A$ and $X^*AX=A$ for complex matrices from a geometric perspective. Although Edelman's work is closely related to our proposed research, their assumption of a non-singular coefficient matrix $A$ differs from our aim to address a general $A$. However, the classical congruence problem still presents several unexplored critical questions for any $A$ and $B$, stemming from the following:

\begin{enumerate}
    \item The matrix congruence question over the field of real numbers.
    \item If we remove the restriction of $X$ being invertible and discuss solutions of the equation $X^tAX=B$.
    \item Consider the special case $X^tAX=A$ where $X \in \mbox{M}_n(k)$.
    \item Study $V(A,B)$ (and in particular $V(A,A)$) from the aspects of matrix algebraic varieties (algebraic homogeneous spaces).
    \end{enumerate}

Matrix varieties are a central area of research in algebraic geometry and representation theory. The variety of commuting nilpotent matrices serves as an excellent example and has inspired numerous works in combinatorics (e.g., Roger-Ramanujan partitions), number theory, and algebraic geometry. Research on the jet schemes of matrix varieties has also produced many high-quality papers. Recently, researchers have paid significant attention to matrix varieties defined by specific conditions on commutators or other similar properties.

Matrix congruence is a well-established topic in the field of linear algebra, with numerous prominent mathematicians contributing to its rich history. Two matrices, $A$ and $B$, are said to be congruent if there exists an invertible matrix $P$ such that $A=P^tBP$. This classic problem has been primarily addressed using linear algebra techniques and has been largely solved for algebraically closed fields. Our aim is to approach a similar problem using commutative algebra and Lie algebraic tools, which will allow us to generalize over any field $k$ and for any matrix $P$ (not necessarily invertible) with coefficients in $k$. (There are several works by \cite{Teran_Lie}, \cite{Teran_Lie_star}, \cite{Teran_Lie_Star_two}, \cite{Teran_orbits} to be cited). One can read the excellent paper \cite{Teran_history} for the historical perspective behind this topic.

Consider a matrix of $n^2$ indeterminates $X=(x_{ij})$, with columns denoted as $X_i$ for $1 \leq i \leq n$. In the matrix equation $X^tAX=B$, the product results in the equation $X_i^tA X_j = b_{ij}$, where $b_{ij}$ is the $ij$-th entry of $B$. Let us denote this equation by $f_{ij}=X_i^tA X_j - b_{ij}$. Define the ideal $I_{(A,B)} := \langle f_{ij} | 1 \leq i,j \leq n\rangle$ in the $k$-algebra $k[x_{ij}]$, referred to as the congruence ideal, and its associated zero set $V_{(A,B)}=V(I_{(A,B)})$, called the congruence variety. The existence of a solution to the congruence equation can now be framed as determining whether the vanishing locus $V_{(A,B)}$ (of $I_{(A,B)}$) is non-empty or not in the field of interest. If the polynomial $\det(X)$ does not belong to the ideal $I_{(A,B)}$, then there is an invertible matrix $X$ such that $X^tAX=B$, which solves the classical congruence problem over the field $k$.

Moreover, observe that $G_A:=V_{(A,A)}\cap \text{GL}n(k)$ is a group that acts on the zero set $V{(A,B)}$ and also on $V_{(A,A)}$ by left multiplication. Therefore, understanding the structure of the zero set $V_{(A,A)}$ (or equivalently, the structure of $I_{(A,A)}$) and its action on $V_{(A,B)}$ is crucial. To fully determine the group $G_A$, we work with its Lie algebra $\mathfrak{g}_A = \{X \in M_n(k) \mid X^tA + AX = 0\}$. By studying certain topological properties of $\mathfrak{g}_A$, we can relate $\text{exp}(\mathfrak{g}_A)$ with $G_A$.
The theory of linear algebraic monoids is an interesting and emerging field of research \cite{Putcha}, \cite{Renner}. The set of matrices $X$ such that $X^tAX=A$ is naturally a linear algebraic monoid. There have not been many studies regarding this class of monoids arising in this fashion. The authors in this article have decided to call such monoids to be ``the congruence monoids". The aim of this paper is to study such monoids when they coincide with their group of units. Apart from the apparent case when the ``coefficient matrix" is invertible we have classified the case when this monoid coincides with the unit group when the coefficient matrix is assumed to be nilpotent. Such monoids arising out of matrix equations are also studied in other articles, namely in \cite{Complex_case} the authors have considered the equation $G^*JG=J$ and described the geometry of the set of solutions. In the paper \cite{integer}, the authors calculated the number of solutions of a general congruence problem and calculated the number of solutions coming from a finite ring.

The matrix varieties, namely the algebraic sets associated with matrix equations, are an important field of study in linear algebra and algebraic geometry. The determinantal varieties play an important role in this area. One of the most famous among these is the variety of commuting matrices. It has been studied by many authors from various angles and multiple connections with other areas have been explored. In \cite{Commuting-nilp-irr2}, the authors demonstrate the irreducibility of the commuting variety when intersected with the variety of the nilpotent matrices. Various authors have discussed the irreducibility \cite{Commuting_nilp-irr} in further generality. In \cite{Commuting-Hilb} the authors have explored relations of commuting varieties with the Hilbert schemes of points. The authors in \cite{Commuting-uppertriangular}, the variety of commuting matrices when restricted to the affine space of the triangular matrices have been studied and they found when these varieties are complete intersections and endowed with other geometric properties. The study of commuting matrices gave rise to so much of activities that there are numerous generalizations and parallel questions \cite{Anti-commuting} for the case of the anti-commuting, the question posed in a tropical set up \cite{Commuting-tropical} have been discussed.
\vspace{1 in}

Simultaneous similarity or simultaneous equivalence is an important problem in linear algebra and representation theory \cite{wild}. The question of matrix pencil equivalence is a particular case of the problem with a large body of mathematics devoted to it. Here let us recall the outline of the classification of matrix pencils up to equivalence and its impact on the congruence problem of matrices. \\
\\

{\bf Question: \cite{Simultaneous}} (Simultaneous equivalence of matrices) For $\{(A_1, \ldots, A_d) \ | \ A_i \in M_n(k)\} = \mathcal{X}$, consider the action of $GL_n(k)$ (or $GL_n(k) \times GL_n(k))$ on $\mathcal{X}$ by $g \ast (A_1, \ldots, A_d) = (gA_1 g^{-1}, \ldots, g A_d g^{-1})$ (or by $(g, h) \ast (A_1, \ldots, A_d) = (gA_1h, \ldots, g A_dh)$). Then, classify the orbits of this action.\\

 {\bf Lemma:} If $X \sim Y$ (there exist $P, Q \in GL_n$ such that $X = PYQ$) both symmetric or skew symmetric, then $X$ and $Y$ are congruent (there exist $H \in GL_n$ such that $X = H^tYH$).\\
    \\
    {\bf Lemma:} For $A, B \in M_n(\mathbb{C})$ we have $A$ is congruent to $B$ if and only if pencils $\mu A + \lambda A^t$ and $\mu B + \lambda B^t$ are equivalent. \\
    \\
   
The aim of this paper is to understand the congruence classes and their direct sum given by TB in more detail by addressing the following things:
\begin{itemize}
\item giving criteria to check which class of matrices forms a group
    \item providing a simpler representative of each class 
    \item understanding the algebraic structure of the group and study its topological properties.
\end{itemize} 




We assume the field is algebraically closed for the following theorem, as we will use the Jordan-Chevalley decomposition. Let us write a matrix $A$ as a sum of its diagonal part and nilpotent part as $A_d+ A_n$.
\begin{lemma}\label{jordan_chevalley_one}
    Let $N$ be a nilpotent triangular matrix (either upper or lower), for any vector $v$, $Nv=N^tv$ if and only if $v \in ker(N) \cap ker(N^t)$.`
\end{lemma}
\begin{proof}
    We choose a basis for the vector space, so that the nilpotent matrix $N$ is in its canonical form. That is with respect to this basis the matrix is of the form, 
    $\begin{bmatrix}
        M_{n_1} & 0 & 0 \cdots 0\\
        0 & M_{n_2} & 0 & 0 \cdots 0\\
        \vdots \vdots \cdots \vdots \\
        0 & 0 & \cdots & M_{n_k}
    \end{bmatrix}$
\end{proof}

\begin{theorem}
Let $A=A_d+A_n$ be a matrix, the monoid $Sol_A$ is a group if and only if $A_d$ restricted to $ker(A_n) \cap ker(A_n^t)$ is non-singular and $Sol_{A_n}$ is a group.
\end{theorem}
\begin{proof}
We know that $Sol_A$ is a group if an only if $ker(A) \cap ker(A^t)$ contains only the trivial vector. Let $v$ be a vector such that $v \in ker(A) \cap ker(A^t)$, then $A_d v+ A_nv =0 = A_dv A_n^tv$. As a result, we have $A_nv=A_n^tv$, now by the Lemma \ref{jordan_chevalley_one}, we know that $v \in ker(A_n) \cap ker(A_n^t)$. As a result we have $ker(A)\cap ker(A^t) = ker(A_n) \cap ker(A_n^t) \cap ker(D)$. So if $Sol_A$ is a group, we have $ker(A) \cap ker(A^t)$ is trivial, this means that the intersection $ker(A_n) \cap ker(A_n^t) \cap ker(A_d)$ is trivial which together with the condition that $A_d$ is non-singular on the $ker(A_n) \cap ker(A_n)^t$ gives that $Sol_{A_n}$ is a group. If $D$ is non-singular then it is clear that $Sol_A$ is a group. For the other direction, if $A_d$ is non-singular, then it is clear that $Sol_A$ is a group, so le us assume that $A_d$ is non-singular on $ker(A_n) \cap ker(A_n^t)$ and $Sol_{A_n}$ is a group. 
\end{proof}

 It is essential that the matrices are congruent. For example the matrix $N$ has the Jordan form $J={\footnotesize\begin{pmatrix}
    0 & 1\\
    0 & 0
\end{pmatrix}}$, one can see that $Sol_N$ is not a group but $Sol_J$ is a group. 



Using the above one can write down an element of the group explicitly as in the following example.
\begin{example}
    Let us consider $n=12$, so the subgroup $N$, has the structure given by the following matrix,  $X = {\tiny\begin{pmatrix}
1&0&x_1&0 & x_2&0\\
0&1&0&0&0&0\\
0& 0&1&0& x_1 & 0\\
0 & -x_1^t & 0 & 1 & 0& 0\\
0&0 & 0& 0 & 1 & 0 \\
0 & -x_2^t+ x_1^{2t} & 0& -x_1^t & 0& 1
\end{pmatrix} }$
where $x_1,x_2 \in M_2(K).$ And, Let $t \in D$. We can write, $t = {\tiny\begin{pmatrix}
s & 0& 0&0 &0 &0\\
0&s^{-t} &0&0 &0 &0\\
0&0&s&0 &0 &0\\
0&0&0&s^{-t} & 0 &0\\
0 & 0 & 0& 0& s & 0\\
0 & 0 & 0 & 0 & 0 & s^{-t}
\end{pmatrix}}$
So now we can write a general element of the group can be written as an element from a general coset, which yields,
{\tiny $$\begin{pmatrix}
s&0&sx_1&0 & sx_2&0\\
0&s^{-t}&0&0&0&0\\
0& 0&s&0& sx_1 & 0\\
0 & -s^{-t}x_1^t & 0 & s^{-t} & 0& 0\\
0&0 & 0& 0 & s & 0 \\
0 & -s^{-t}x_2^t+ s^{-t}x_1^{2t} & 0& -s^{-t}x_1^t & 0& s^{-t}
\end{pmatrix}$$}
If we rewrite and replace the matrices $sx_1,sx_2$ by simply $x_1,x_2$, we obtain the following expression for a general element of the group.\\
{\tiny \[\begin{pmatrix}
s&0&x_1&0 & x_2&0\\
0&s^{-t}&0&0&0&0\\
0& 0&s&0& x_1 & 0\\
0 & -s^{-t}x_1^ts^{-t} & 0 & s^{-t} & 0& 0\\
0&0 & 0& 0 & s & 0 \\
0 & -s^{-t}x_2^ts^{-t}+ s^{-t}x_1^{2t}s^{-2t} & 0& -s^{-t}x_1^ts^{-t} & 0& s^{-t}
\end{pmatrix}\]}
\end{example}

he idea is the following: if the entry is zero in Lie algebra, then we can have constants in the Lie group but that is also not possible because in that case, the matrix $X$ won't satisfy $X^tA_n^2X = A_n^2$. Thus the corresponding entry in the Lie group also has to be zero. Furthermore, for a non-zero entry in Lie algebra, we take the linear part of the equations from the Lie algebra of the subgroup $N$ and introduce non-linear parts.

 (singular subspaces or, in general, subspaces of matrices with bounded rank), which are an essential field of linear algebra. One can find important information regarding these in \cite{singular_one}, \cite{singular_two}, \cite{singular_three}, and in the references thereof).

 Observe that, if $G$ is an algebraic group $G_u$ is the unipotent radical of it and $G_r$ is the reductive quotient. If $G$ acts on an affine variety $X$ and let the action of $G$ on the algebra of regular functions $k[X]$ be the natural action obtained through it, then the invariants of $G$ and that of $G_u$ and $_r$ are related in the following manner, $k[X]^G= (k[X]^{G_r})^{G_u}$. So in our situation, for $G=Sol_{A_n}$ (or $Sol_{A_n}^2$), one can concentrate on the unipotent part of the groups to find the invariants as the Nagata, Haboush theorem thoroughly covers the reductive part.
 
